Optimization of Embedded Element Patterns of Reactively Loaded Antenna Arrays

This paper introduces a framework for synthesizing reactively loaded antennas and antenna arrays. The framework comprises two main components: computing the fundamental bound using the semi-definite relaxation and finding a realizable solution via optimization on a Riemannian manifold. The embedded element patterns are subject to the optimization with two distinct goals under study: focusing the radiation in a single direction or synthesizing patterns with desired shapes. The reactive terminations of passive antenna elements serve as optimization variables. We demonstrate the framework using a connected bowtie-slot antenna and antenna array with both beam-focusing and beam-shaping targets. The tests show that the optimization on the Riemannian manifold yields superior results compared to existing methods, such as the genetic algorithm. This is particularly evident in the most complex and extensive problem, which requires the synthesis of shaped embedded element patterns for a sparse reactively loaded antenna array with a limited field of view.

==> Figures/complexity/complexity.tex <==
\begin{tikzpicture}

% let both axes use the same layers
% \pgfplotsset{set layers}

\begin{axis}[%'
name={COMP_TIME_N3},
width=3.75cm,
height=4.5cm,
title={$\ND = 3$},
every axis title/.style={below, at={(0.5,1)},draw=black,fill=white},
axis y line*=left,
at={(0,0)},
xmin=5,
xmax=60,
xlabel={$\NP$},
ymin=0,
ymax=300,
ylabel={time (s)},
ylabel shift = -0.15cm,
xlabel shift = -0.1cm,
xtick = {10, 30, 50},
xmajorgrids,
ymajorgrids,
grid style={dashed, cap=round, dash pattern = on 0.5mm off 0.375mm, line width=1/4, opacity=0.5},
axis background/.style={fill=white},
axis line style={solid, line width=0.5pt},
]

\addplot[line width=1.25pt, PairedJ, cap=round, join=round] table[col sep=comma]{Figures/complexity/t_sdr_N3.txt};
\label{COMP_TIME_N3:SDR}

\addplot[ManuOpt] table[col sep=comma]{Figures/complexity/t_mo_N3.txt};
\label{COMP_TIME_N3:MO}

\addplot[GA] table[col sep=comma]{Figures/complexity/t_ga_N3.txt};
\label{COMP_TIME_N3:GA}

\addplot[line width=1.75pt, gray, cap=round, join=round, smooth] table[col sep=comma]{Figures/complexity/t_tot_N3.txt};
\label{COMP_TIME_N3:TOT}

\addplot[resultEEP2, line width=0.75pt] table[col sep=comma]{Figures/complexity/t_fit_N3.txt};
\label{COMP_TIME_N3:FIT}

\end{axis}

\begin{axis}[%
name={COMP_COST_N3},
width=3.75cm,
height=4.5cm,
axis y line*=right,
yticklabel=\empty,
axis x line=none,
xmin=5,
xmax=60,
at={(0,0)},
ymin=0,
ymax=400,
% ylabel={cost},
% ylabel shift = -0.15cm,
% xlabel shift = -0.1cm,
% xtick = {10, 30, 50},
% xmajorgrids,
% ymajorgrids,
% grid style={dashed, cap=round, dash pattern = on 0.5mm off 0.375mm, line width=1/4, opacity=0.5},
% axis background/.style={fill=white},
axis line style={solid, line width=0.5pt},
]

\addplot[line width=1.25pt, PairedJ, cap=round, join=round, densely dashed] table[col sep=comma]{Figures/complexity/cost_sdr_N3.txt};
\label{COMP_COST_N3:SDR}

\addplot[ManuOpt, densely dashed] table[col sep=comma]{Figures/complexity/cost_mo_N3.txt};
\label{COMP_COST_N3:MO}

\addplot[GA, densely dashed] table[col sep=comma]{Figures/complexity/cost_ga_N3.txt};
\label{COMP_COST_N3:GA}

\end{axis}

% SECOND PLOT
\begin{axis}[%
name={COMP_TIME_N4},
width=3.75cm,
height=4.5cm,
title={$\ND = 4$},
every axis title/.style={below, at={(0.5,1)},draw=black,fill=white},
yticklabel=\empty,
axis y line*=left,
at={(COMP_COST_N3.right of south east), anchor=right of south west},
xshift=-0.1cm,
xmin=5,
xmax=60,
xlabel={$\NP$},
ymin=0,
ymax=300,
% ylabel={computing time (s)},
% ylabel shift = -0.15cm,
xlabel shift = -0.1cm,
xtick = {10, 30, 50},
xmajorgrids,
ymajorgrids,
grid style={dashed, cap=round, dash pattern = on 0.5mm off 0.375mm, line width=1/4, opacity=0.5},
axis background/.style={fill=white},
axis line style={solid, line width=0.5pt},
]

\addplot[line width=1.25pt, PairedJ, cap=round, join=round] table[col sep=comma]{Figures/complexity/t_sdr_N4.txt};
\label{COMP_TIME_N4:SDR}

\addplot[ManuOpt] table[col sep=comma]{Figures/complexity/t_mo_N4.txt};
\label{COMP_TIME_N4:MO}

\addplot[GA] table[col sep=comma]{Figures/complexity/t_ga_N4.txt};
\label{COMP_TIME_N4:GA}

\addplot[line width=1.75pt, gray, cap=round, join=round, smooth] table[col sep=comma]{Figures/complexity/t_tot_N4.txt};
\label{COMP_TIME_N4:TOT}

\addplot[resultEEP2, line width=0.75pt] table[col sep=comma]{Figures/complexity/t_fit_N4.txt};
\label{COMP_TIME_N4:FIT}

\addplot[line width=1.25pt, black, cap=round, join=round, smooth] table[]{
A B
0 5000
};
\label{COMP_TIME:BLACK}

\addplot[line width=1.25pt, black, cap=round, join=round, smooth, densely dashed] table[]{
A B
0 5000
};
\label{COMP_COST:BLACK}

\begin{pgfonlayer}{foreground layer}
	\node[draw,fill=white,draw=black,cap=round, fill opacity=0.95] at (axis cs: 27.5, 350) [anchor=south] {\begin{tabular}{cccc}
			\addlinespace[-0.2em]\ref{COMP_TIME:BLACK} & time \quad & \ref{COMP_COST:BLACK} & cost \\[-0.6em]
	\end{tabular}};
\end{pgfonlayer}

\begin{pgfonlayer}{foreground layer}
	\node[draw,fill=white,draw=black,cap=round, fill opacity=0.95] at (axis cs: 27.5, 315) [anchor=south] {\begin{tabular}{cccccccccc}
			\addlinespace[-0.2em]\ref{COMP_TIME_N4:SDR} & bound \quad & \ref{COMP_TIME_N4:MO} & MO \quad & \ref{COMP_TIME_N4:TOT} & bound + MO \quad & \ref{COMP_TIME_N4:FIT} & fitted \quad & \ref{COMP_TIME_N4:GA} & GA \\[-0.6em]
	\end{tabular}};
\end{pgfonlayer}

\end{axis}

\begin{axis}[%
name={COMP_COST_N4},
width=3.75cm,
height=4.5cm,
axis y line*=right,
yticklabel=\empty,
axis x line=none,
xmin=5,
xmax=60,
at={(COMP_COST_N3.right of south east), anchor=right of south west},
xshift=-0.1cm,
ymin=0,
ymax=400,
% ylabel={cost},
% ylabel shift = -0.15cm,
% xlabel shift = -0.1cm,
% xtick = {10, 30, 50},
% xmajorgrids,
% ymajorgrids,
% grid style={dashed, cap=round, dash pattern = on 0.5mm off 0.375mm, line width=1/4, opacity=0.5},
% axis background/.style={fill=white},
axis line style={solid, line width=0.5pt},
]

\addplot[line width=1.25pt, PairedJ, cap=round, join=round, densely dashed] table[col sep=comma]{Figures/complexity/cost_sdr_N4.txt};
\label{COMP_COST_N4:SDR}

\addplot[ManuOpt, densely dashed] table[col sep=comma]{Figures/complexity/cost_mo_N4.txt};
\label{COMP_COST_N4:MO}

\addplot[GA, densely dashed] table[col sep=comma]{Figures/complexity/cost_ga_N4.txt};
\label{COMP_COST_N4:GA}

\end{axis}


% THIRD PLOT
\begin{axis}[%
name={COMP_TIME_N5},
width=3.75cm,
height=4.5cm,
title={$\ND = 5$},
every axis title/.style={below, at={(0.5,1)},draw=black,fill=white},
yticklabel=\empty,
axis y line*=left,
at={(COMP_COST_N4.right of south east), anchor=right of south west},
xshift=-0.1cm,
xmin=5,
xmax=60,
xlabel={$\NP$},
ymin=0,
ymax=300,
% ylabel={computing time (s)},
% ylabel shift = -0.15cm,
xlabel shift = -0.1cm,
xtick = {10, 30, 50},
xmajorgrids,
ymajorgrids,
grid style={dashed, cap=round, dash pattern = on 0.5mm off 0.375mm, line width=1/4, opacity=0.5},
axis background/.style={fill=white},
axis line style={solid, line width=0.5pt},
]

\addplot[line width=1.25pt, PairedJ, cap=round, join=round] table[col sep=comma]{Figures/complexity/t_sdr_N5.txt};
\label{COMP_TIME_N5:SDR}

\addplot[ManuOpt] table[col sep=comma]{Figures/complexity/t_mo_N5.txt};
\label{COMP_TIME_N5:MO}

\addplot[GA] table[col sep=comma]{Figures/complexity/t_ga_N5.txt};
\label{COMP_TIME_N5:GA}

\addplot[line width=1.75pt, gray, cap=round, join=round, smooth] table[col sep=comma]{Figures/complexity/t_tot_N5.txt};
\label{COMP_TIME_N5:TOT}

\addplot[resultEEP2, line width=0.75pt] table[col sep=comma]{Figures/complexity/t_fit_N5.txt};
\label{COMP_TIME_N5:FIT}

\end{axis}

\begin{axis}[%
name={COMP_COST_N5},
width=3.75cm,
height=4.5cm,
axis y line*=right,
axis x line=none,
xmin=5,
xmax=60,
at={(COMP_COST_N4.right of south east), anchor=right of south west},
xshift=-0.1cm,
ymin=0,
ymax=400,
ylabel={cost ($\mathrm{V}^2 / \mathrm{m}^2$)},
ylabel shift = -0.15cm,
xlabel shift = -0.1cm,
% xtick = {10, 30, 50},
% xmajorgrids,
% ymajorgrids,
% grid style={dashed, cap=round, dash pattern = on 0.5mm off 0.375mm, line width=1/4, opacity=0.5},
% axis background/.style={fill=white},
axis line style={solid, line width=0.5pt},
]

\addplot[line width=1.25pt, PairedJ, cap=round, join=round, densely dashed] table[col sep=comma]{Figures/complexity/cost_sdr_N5.txt};
\label{COMP_COST_N5:SDR}

\addplot[ManuOpt, densely dashed] table[col sep=comma]{Figures/complexity/cost_mo_N5.txt};
\label{COMP_COST_N5:MO}

\addplot[GA, densely dashed] table[col sep=comma]{Figures/complexity/cost_ga_N5.txt};
\label{COMP_COST_N5:GA}

\end{axis}

\end{tikzpicture}%
